Efficient Proton Transport Modelling for Proton Beam Therapy and Biological Quantification

In this work, we present a fundamental mathematical model for proton transport, tailored to capture the key physical processes underpinning Proton Beam Therapy (PBT). The model provides a robust and computationally efficient framework for exploring various aspects of PBT, including dose delivery, linear energy transfer, treatment planning and the evaluation of relative biological effectiveness. Our findings highlight the potential of this model as a complementary tool to more complex and computationally intensive simulation techniques currently used in clinical practice.

==> Figures/Lung.tex <==
or bragg kleeman for proton therapy\begin{tikzpicture}[scale=0.6]
    \definecolor{skinColor}{RGB}{255,224,189}
    \definecolor{adiposeColor}{RGB}{255,240,227}
    \definecolor{muscleColor}{RGB}{205,155,155}
    \definecolor{boneColor}{RGB}{216,191,216}
    \definecolor{lungColor}{RGB}{173,216,230}
    \definecolor{tumourColor}{RGB}{205,92,92}
    
    % Layers
    \draw[fill=skinColor] (0,0) rectangle (0.3,10);
    \node[rotate=90, font=\tiny] at (0.15,5) {Skin $\rho = 1.09$ g/cm$^3$};
    
    \draw[fill=adiposeColor] (0.3,0) rectangle (1.8,10);
    \node[rotate=90, font=\small] at (1,5) {Adipose Tissue $\rho = 0.92$ g/cm$^3$};
    
    \draw[fill=muscleColor] (1.8,0) rectangle (3.3,10);
    \node[rotate=90, font=\small] at (2.5,5) {Muscle $\rho = 1.04$ g/cm$^3$};
    
    \draw[fill=boneColor] (3.3,0) rectangle (4,10);
    \node[rotate=90, font=\small] at (3.7,5) {Bone $\rho = 1.85$ g/cm$^3$};
    
    \draw[fill=lungColor] (4,0) rectangle (10,10);
    \node[rotate=90, font=\small] at (7,5) {Lung $\rho = 0.3$ g/cm$^3$};
    
    \draw[fill=tumourColor] (10,0) rectangle (13,10);
    \node[rotate=90, font=\small] at (11.5,5) {Tumour $\rho = 1.0$ g/cm$^3$};
    
    \draw[fill=lungColor] (13,0) rectangle (16,10);
    \node[rotate=90, font=\small] at (14.5,5) {Lung $\rho = 0.3$ g/cm$^3$};
    
    \draw[fill=boneColor] (16,0) rectangle (16.7,10);
    \node[rotate=90, font=\small] at (16.35,5) {Bone $\rho = 1.85$ g/cm$^3$};
    
    \draw[fill=muscleColor] (16.7,0) rectangle (18.2,10);
    \node[rotate=90, font=\small] at (17.45,5) {Muscle $\rho = 1.04$ g/cm$^3$};
    
    \draw[fill=adiposeColor] (18.2,0) rectangle (19.7,10);
    \node[rotate=90, font=\small] at (18.95,5) {Adipose Tissue $\rho = 0.92$ g/cm$^3$};
    
    \draw[fill=skinColor] (19.7,0) rectangle (20,10);
    \node[rotate=90, font=\tiny] at (19.85,5) {Skin $\rho = 1.09$ g/cm$^3$};
    
    % Labels
    \node at (10,-2) {Depth (cm)};

    % Depth ticks
    \foreach \x in {0,1,...,20} {
      \draw (\x,-0.5) -- (\x,0);
      \node at (\x, -1) {\small \x};
    }   
  \end{tikzpicture}
